Measurement of ${\sigma(H\nu_e\bar{\nu_e})\times BR(H\rightarrow ZZ^\ast)}$ and Higgs production in $ZZ$ fusion at a 1.4 TeV CLIC collider

This paper presents the potential measurement at 1.4 TeV CLIC of the cross-section (times branching ratio) of the Higgs production via $WW$ fusion with the Higgs subsequently decaying in $ZZ^\ast$, ${\sigma(H\nu_e\bar{\nu_e})\times BR(H\rightarrow ZZ^\ast)}$, and of the Higgs production via $ZZ$ fusion with the Higgs subsequently decaying in $b\bar{b}$, ${\sigma(He{^+}e{^-})\times BR(H\rightarrow b\bar{b})}$. For the $H\rightarrow ZZ^\ast$ decay the hadronic final state, ${ZZ^\ast\rightarrow q\bar{q}q\bar{q}}$, and the semi-leptonic final state, ${ZZ^\ast\rightarrow q\bar{q}l^+l^-}$, are considered. The results show that ${\sigma(H\nu_e\bar{\nu_e})\times BR(H\rightarrow ZZ^\ast)}$ can be measured with a precision of 18.3% and 6% for the hadronic and semi-leptonic channel, respectively. ${\sigma(He{^+}e{^-})\times BR(H\rightarrow b\bar{b})}$ can be measured with a precision of 1.7%. This measurement also contributes to the determination of the Higgs coupling to the $Z$ boson, $g_{H_{ZZ}}$.

==> conclusions.tex <==

There is a strong motivation to use precise Higgs measurements at \ac{CLIC} to search for physics beyond the Standard Model. 
The measurement of Higgs boson couplings are of particular interest. 
The measurement of the branching ratio for the rare \ac{SM}-like Higgs decay into two muons was simulated at a 1.4 CLIC collider with unpolarised beams. The measurement itself tests the muon identification and momentum resolution of the detector. 

It was shown that the measurement of the cross-section times the branching ratio for the Standard Model Higgs decay into two muons can be performed with a statistical uncertainty of 38\percent, assuming 1.5~\abinv integrated luminosity with unpolarized beams. If the same integrated luminosity is collected with 80\percent left-handed polarisation for the electrons and 30\percent right handed polarisation for the positrons, the statistical uncertainty improves to beter than 25\%. The systematic uncertainties are negligible in comparison. The largest contributions to the statistical uncertainty come from the limited statistics of the signal and from the presence of the signal-like backgrounds from \nnmm and \ggnnmm processes. The uncertainty of \sigmaBR of 38\percent translates into the uncertainty of Higgs coupling to muons, \gHMuMu, of \couplingunc\percent.


==> event_selection.tex <==
In both final states, fully hadronic and semi-leptonics, the event selection is done in several steps. First, a preselection between signal and background events is performed using
cuts. Then, the final event selection uses a multivariate classifier based on boosted decision trees. For the semi-leptonic final state, 
there is one more step, a post-selection, which is introduced in order to suppress $e^-e^+\rightarrow H\nu\bar{\nu}, H\rightarrow \PW\PW, \PW\PW\rightarrow qqqq$ and $e^-e^+\rightarrow H\nu\bar{\nu}, H\rightarrow b\bar{b}$
processes and which does not have influence of the signal efficiency.






==> event_selectionbb.tex <==
In both final states, fully hadronic and semi-leptonics, the event selection is done in several steps. First, a preselection between signal and background events is performed using
cuts. Then, the final event selection uses a multivariate classifier based on boosted decision trees. For the semi-leptonic final state, 
there is one more step, a post-selection, which is introduced in order to suppress $e^-e^+\rightarrow H\nu\bar{\nu}, H\rightarrow \PW\PW, \PW\PW\rightarrow qqqq$ and $e^-e^+\rightarrow H\nu\bar{\nu}, H\rightarrow b\bar{b}$
processes and which does not have influence of the signal efficiency.





